Non-intrusive inference reduced order model for fluids using linear multistep neural network

In this effort we propose a data-driven learning framework for reduced order modeling of fluid dynamics. Designing accurate and efficient reduced order models for nonlinear fluid dynamic problems is challenging for many practical engineering applications. Classical projection-based model reduction methods generate reduced systems by projecting full-order differential operators into low-dimensional subspaces. However, these techniques usually lead to severe instabilities in the presence of highly nonlinear dynamics, which dramatically deteriorates the accuracy of the reduced-order models. In contrast, our new framework exploits linear multistep networks, based on implicit Adams-Moulton schemes, to construct the reduced system. The advantage is that the method optimally approximates the full order model in the low-dimensional space with a given supervised learning task. Moreover, our approach is non-intrusive, such that it can be applied to other complex nonlinear dynamical systems with sophisticated legacy codes. We demonstrate the performance of our method through the numerical simulation of a two-dimensional flow past a circular cylinder with Reynolds number Re = 100. The results reveal that the new data-driven model is significantly more accurate than standard projection-based approaches.

==> Untitled_Document <==
Designing an accurate and efficient reduced order model for nonlinear fluid dynamics is a challenging problem for many realistic engineering applications. The classic Galerkin projection based reduced order model (GP-ROM) has the projection stability error which inaccurately approximates the nonlinear dynamics. We propose a novel multi-step neural network inference reduced order model (MNNI-ROM) for the numerical simulation of fluid flows. The new MNNI-ROM uses a neural network discretize the low dimension ROM dynamics by using linear multi-time stepping method. The ROM dynamics is then trained from the multistep neural network. The new MNNI-ROM that is fully learned from the data without intrusively using any operator from the full model. We investigate the MNNI-ROM in the numerical simulation of a 2D channel flow past a circular cylinder at Reynolds number Re = 100. The MNNI-ROM is significantly more accurate than the classic Galerkin projection ROM (GP-ROM).

The increasing need for accurate identification and prediction of complex fluid systems are often resulting in the numerical simulation and analyze a large-scale nonlinear dynamical system. It puts an overwhelming demand and a heavy burden on the computational resources, especially if repeated model evaluations over a large range of parameter values are required, which makes it prohibitive to use the original system. Reduced order modeling of fluid dynamic system seeks to construct a reduced order model (ROM) with orders of magnitude reduction in computational complexity as well as the accurate approximation of the full model. Reduced order models (ROMs) have tremendous applications in system identification and prediction, control design, optimization etc.

The classic Galerkin projection based ROM (GP-ROM) is one of the most successful models and has been widely applied to realistic engineering fluid problems. The GP-ROM constructs a low-dimensional space using data reduction method and then projects the equations of the full order model (original system) onto the reduced space to obtain the reduced nonlinear dynamic system. The reduced nonlinear dynamic system is often constructed intrusively via Galerkin projection of the full model operators, which means the full order model operators have to be available in the reduced order model derivation. This limits the applicability of projection based model reduction in many situations where the full model is unknown.

Another drawback of the GP-ROM is the inaccuracy by the numerical instability for many nonlinear fluid problems. This instability comes from the truncation process of the reduced space. The low dimension (reduced) space is often generated by proper orthogonal decomposition (POD) method, also known as principal component analysis (PCA). This method truncates the eigenvectors corresponding to the largest eigenvalues of the full order model data. The reduced space formed by POD basis extracts the most pertinent features of the data set and makes the GP-ROM very efficient because the rank of the reduced space is generally the order of 10 compared to the high dimension of the full order model. However, the reduced space causes a significant loss of information due to the truncation process, which makes the GP-ROM inaccurately approximate the full model especially for a highly non-stationary fluid system, i.e., turbulence. In the ROM literature, a common explanation for this failure is that the GP-ROM fail to account for energy transfer from resolved to unresolved POD modes because of the truncation. This also limits the applicability of GP-ROM. There have been considerable efforts to alleviate this drawback by modeling the discarded information both physically and mathematically, known as ROM closure modeling.


Numerous models for the ROM closure problem have been devised to address the numerical instability. The stabilization strategies often come from two ways. 
One is based on phenomenological arguments that modeling the physical effect of the lost information by adding physical viscosity to the ROM. Another approach is data-driven modeling the discarded POD modes by using the data and mathematical equations of the full order model. Ofen an optimization problem has to be solved for the closure problem. Recently, neural network has also been introduced to approximate the truncated POD modes in the GP-ROM. All these models belong to the wide class of stabilization GP-ROM. On the other hand, the construction of stabilization GP-ROM cannot avoid the intrusive projection step which, as mentioned before, limit the applicability. Recently, non-intrusive model reduction method using a second order Taylor series and Smolyak sparse grid collocation method to calculate the ROM coefficients for Navier-Stokes equations (NSE) has been introduced. Peherstorfer used a nonintrusive operator inference method for ROM was introduced, which approximate the ROM dynamic system by using a second order operator and solving the related least square optimization problem to obtain the operator. However, practical considerations such as the ill-conditioned matrix for the optimization problem and predictability have to be made especially for complex fluid system e.g., high Reynolds number fluid flows. With the recent development in supervised deep learning, the data-driven discovery of complex dynamic systems has emerged as a prominent research field. Several deterministic and probabilistic models with neural network, Gaussian process have been developed for identifying nonlinear dynamics. Rasi introduced the multistep neural network for multiple systems prediction and identification. 

In this paper, we introduce a novel approach to the nonintrusive reduced-order modeling of fluid dynamics that combines the classical multistep family of time-stepping schemes with deep neural networks. This new ROM can overcome the aforementioned drawbacks of GP-ROM by using a multistep neural network. Unlike other nonintrusive ROM method and stabilization GP-ROM, the multistep neural network inference ROM (MNNI-ROM) use data to learn the ROM dynamics which circumvent some practical issues from other methods. Also, the MMNI-ROM has advantages over the GP-ROM by addressing the instability problem from the learning. We test our new MNNI-ROM on the golden standard benchmark fluid problem, i.e., 2D flow past a cylinder. The numerical results demonstrate that our new MNNI-ROM provides accurate approximation and prediction while maintaining low computational cost. Another advantage is that the new approach does not have to have direct access or approximations to temporal gradients because the time derivatives are discretized using classical time-stepping methods.

In this section, we present the architecture of the ROM dynamics inference using multistep neural newtwork. In contrast to the classic GP-ROM framework, we consider the low dimensional ROM dynamic system as a general functional. This general functional $f$ contains linear ($L$), second order ($N$), and high order terms (e.g., $\btau$ but not restricted to) to the ROM dynamics that approximate the full model. Our goal is to infer the dynamic dependecies in a given set of temporal data, and return a closed form model that approximate the full model and also can be subsequently used to forecast future states.

In numerical analysis, the classic linear multistep method for ODE system use information from the previous K steps to calculate the next value. It has a form of the following:

Different choices for the parameters $\alpha_K$ and $\beta_K$ result in specific schemes. It turns to the famous trapezoidal rule.

\textbf{Multistep Neural Network (MNN).} 
Dynamic neural networks (e.g., RNN, LSTM) have been widely used for system identification \cite{narendra1990identification,chen1992neural}. The MNN was first introduced by \citeauthor{raissi2018multistep} (2018). It constructs a structured nonlinear regression model that combines family of multistep schemes and neural network to infer the ROM dynamics. Given the dataset of $\ba(t)$ for system \eqref{eqn:rom-dy} at several time instances, $t_0,t_1,...,t_s$, we proceed by placing a nueural netowrk prior on the functional $f$ using linear multistep method. The parameters of this neural network can be learned by minimizing the mean squared error loss function:
\begin{eqnarray}
\label{eqn:nn-lost}
MSE: = \frac{1}{N - K + 1}\sum_{n=K}^N|\mathbf{y}_n|^2
\end{eqnarray}
$\mathbf{y}_n$, defined as following, can be obtained from the family of multistep time-stepping scheme \eqref{eqn:lm-method},
\begin{eqnarray}
\label{eqn:nn-lost-y}
\mathbf{y}_n:=\sum_{i=0}^K[\alpha_i\ba_{n-i} + \Delta t \beta_if(\ba_{n-i})],\,\,\, n = K,...,S
\end{eqnarray}
Where $K$ is the steps of the linear multistep method and $S$ is the total number of time instance in the ROM dynamic system. One advantage of this regression is that we do not have to approximate the temporal gradients \cite{peherstorfer2016data} since the time derivatives are discretized by the multistep method.

\textbf{MNN Inference ROM.} We use the trained neural network to infer the ROM dynamic system \eqref{eqn:rom-dy} and approximate the full model of NSE.  We claim that the performance of the learned ROM dynamics is much better than the classic GP-ROM in approximation of NSE and prediction.
We emphasize that the novelty of our MNNI-ROM is the non-instrusively learning of the reduced ROM system from data, whereas GP-ROM and closure modeling require the use of full model operator. Fig.\ref{fig-nnirom-pic} shows the difference between MNNI-ROM and classic GP-ROM.
\begin{figure}[h!]
              \includegraphics[width=\linewidth]{MNI.png}
              \caption{diagram of intrusive projection based model reduction and the new neural network inference model reduction}
\label{fig-nnirom-pic}
\end{figure}

\subsection{Dataset}
The input of this neural network is the time-varying POD coefficients in \eqref{eqn:g-rom-1}, which can be obtained by projecting the data to the reduced space. Let $\bU=\bu^0,...,\bu^s\in \mathcal{R}^{D_h\times{s+1}}$ be the data matrix of the discrete solutions of the NSE system \eqref{eqn:nse-1} at time step $t_0,...,t_s$, and $\bu^0$ is the initial condition. After constructed the reduced space $\Phi_r=\{\varphi_i\}_{i=1}^r$, we use eqn.(\ref{eqn:rom-proj}) to project our data onto the POD space to obtain the trajectory of the POD coefficients 
\begin{eqnarray}
\label{eqn:rom-proj}
(\bu^j, \varphi_k) = (\sum_{i=1}^ra^j_i\varphi_i,\varphi_k)
\end{eqnarray}
$k,i=1,2,..,r$ and $j=t_0,t_1,..,t_s$. By using the orthogonality of the POD basis, we can get the following matrix form of the projection:
\begin{eqnarray}
\label{eqn:training-mat}
I_rA = \Phi_r^TW\bU
\end{eqnarray}
Where $I_r\in \mathcal{R}^{r\times r}$ is the identity matrix , $W\in\mathcal{R}^{D_h\times D_h}$ is the weight matrix of the $L^2$ inner product \eqref{eqn:rom-proj}, we use finite element weights in this work. $A=[\ba^0,\ba^1,...,\ba^s] \in \mathcal{R}^{r\times (s+1)}$ is the training dataset for the neural network which represents the trajectory of the time-varying coefficients of the full model data. We outline the framework of the MNNI-ROM in the following:
\begin{algorithm}[H]
	\caption{Multistep Neural Network Inference Reduced Order Model (MNNI-ROM)}
	\label{alg:nni-rom}
	\begin{algorithmic}[1]
		%\Statex{\textbf{Offline:}}
		\State{Compute the reduced POD space from the data of NSE by \eqref{eqn:pod-svd}	
		}
		\State{ Compute the input data matrix $A$ via \eqref{eqn:training-mat}
					}
		\State{
				Train the neural network using loss function \eqref{eqn:nn-lost}
					}		
		 \State{
					The MNNI-ROM for NSE is obatined from the trained low dimension dynamic system:
								\begin{equation}
									\boxed{
									\dot{\ba}=\hat{\bbf}_{NN}(\ba)
									} 
									\label{eqn:mnni-rom-online}
								\end{equation}
					}
\end{algorithmic}
\end{algorithm}
\noindent The construction of the new model does not use any full model operator. The MNNI-ROM framework has the generality that can be applied to reduced order modeling of any nonlinear dynamic system. The main offline computational cost of MNNI-ROM is training the MNN, which depends on the number of neurons, layers and time-steps. Whereas the GP-ROM offline cost is assembly the tensors, $L$, $N$ in \eqref{eqn:g-rom-2}. In general, the GP-ROM offline computation is faster than MNNI-ROM because the assembly of tensors only requre explicit use of projection from full model operator (see \eqref{eqn:g-rom-3b}) which has complexity $\mathcal{O}(r^3)$ and note $r$ is very small. The MNN training is higher considering the hyperparameters tunning in practical, e.g., learning rate, layers, steps. However, the benefit is that once the MNN is trained, the inferred ROM dynamics from the neural network can provide a better  approximation to the full model of NSE than GP-ROM and contain predictability. 



